Tight bounds on the mutual coherence of sensing matrices for Wigner D-functions on regular grids

Many practical sampling patterns for function approximation on the rotation group utilizes regular samples on the parameter axes. In this paper, we relate the mutual coherence analysis for sensing matrices that correspond to a class of regular patterns to angular momentum analysis in quantum mechanics and provide simple lower bounds for it. The products of Wigner d-functions, which appear in coherence analysis, arise in angular momentum analysis in quantum mechanics. We first represent the product as a linear combination of a single Wigner d-function and angular momentum coefficients, otherwise known as the Wigner 3j symbols. Using combinatorial identities, we show that under certain conditions on the bandwidth and number of samples, the inner product of the columns of the sensing matrix at zero orders, which is equal to the inner product of two Legendre polynomials, dominates the mutual coherence term and fixes a lower bound for it. In other words, for a class of regular sampling patterns, we provide a lower bound for the inner product of the columns of the sensing matrix that can be analytically computed. We verify numerically our theoretical results and show that the lower bound for the mutual coherence is larger than Welch bound. Besides, we provide algorithms that can achieve the lower bound for spherical harmonics.

==> Sections/discussions.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussion}
The theoretical and experimental results in this work are derived by considering equispaced sampling points on the elevation $\bs \theta \in \mbb{R}^m$ given in \eqref{ch5:eq equispaced}. In practice, we can optimize the sampling points on the elevation $\bs \theta \in \mbb{R}^m$ by using Algorithm \ref{algo_ps} as well. As a consequence, the gradient of the function on the elevation should be taken into account. For Wigner D-functions, it is equal to the derivative of product Wigner d-functions with respect to the elevation angles. Similarly, for spherical harmonics the derivative of product two associated Legendre polynomials should be evaluated. Using product rule of derivative and the derivative of those functions, we can optimize all angles.

Figure \ref{Fig opt_SH_all} depicts a numerical experiment of this approach on spherical harmonics sensing matrix. It becomes evident that, we can construct pair of sampling points on elevation and azimuth, i.e., $(\theta_p,\phi_p)$ for $p \in [m]$, that yield a sensing matrix with the coherence lower than the bound in Theorem \ref{ch5:thm prod}.  
\begin{figure}[!htb]
\centering
\inputTikZ{0.5}{Figure/GradDescAllThetaPhiSH.tikz}
\caption{Coherence of spherical harmonics sensing matrix ($B = 32)$}
\label{Fig opt_SH_all}
\end{figure}
In this case, the Adam algorithm still performs better than other algorithms. However, as described in the figure, it is still difficult to achieve the Welch bound or the universal lower bound of the coherence \cite{welch_lower_1974}.  
\section{Conclusion and Future Works}\label{sec5}
In this paper, we presented the proof of the maximum product of equispaced samples Wigner d-functions. This problem appears when designing sensing matrices constructed from Wigner D-functions and spherical harmonics. Borrowing tools from angular momentum in quantum mechanics, we can represent the product using angular momentum coefficients, called Wigner 3j symbols. Harnessing properties of those coefficients and carefully choosing sampling points on the elevation, providing guidelines to show that the maximum can be attained at zero-order polynomials, which equals to Legendre polynomials. This bound can be used to design sampling points on the sphere or the rotation group to construct low-coherence sensing matrices. As shown in the numerical evaluations, we can adopt several stochastic gradient descent algorithms to accomplish this purpose. However, another investigation is required whether there is a closed-form construction of deterministic sampling points, independent from the optimization, to achieve the bound.

Since the strategy of the proof relies heavily on the structure of sampling points in the elevation, which is equispaced, this imposes another challenge in this work is, whether we can optimize all angles to have the coherence of the sensing matrix lower than the coherence bound. Numerical experiments showed that, by tailoring the stochastic gradient method, one could design sampling points on the sphere that attain this condition. At the moment, we can not give a theoretical argument about whether the closed-form formula exists. This problem will be relegated in future works.
